Vulnerability of Face Recognition to Deep Morphing

It is increasingly easy to automatically swap faces in images and video or morph two faces into one using generative adversarial networks (GANs). The high quality of the resulted deep-morph raises the question of how vulnerable the current face recognition systems are to such fake images and videos. It also calls for automated ways to detect these GAN-generated faces. In this paper, we present the publicly available dataset of the Deepfake videos with faces morphed with a GAN-based algorithm. To generate these videos, we used open source software based on GANs, and we emphasize that training and blending parameters can significantly impact the quality of the resulted videos. We show that the state of the art face recognition systems based on VGG and Facenet neural networks are vulnerable to the deep morph videos, with 85.62 and 95.00 false acceptance rates, respectively, which means methods for detecting these videos are necessary. We consider several baseline approaches for detecting deep morphs and find that the method based on visual quality metrics (often used in presentation attack detection domain) leads to the best performance with 8.97 equal error rate. Our experiments demonstrate that GAN-generated deep morph videos are challenging for both face recognition systems and existing detection methods, and the further development of deep morphing technologies will make it even more so.

==> sections/relatedwork.tex <==
\section{Related work}
\label{sec:related}

%\begin{figure}[tb]
%\centering
%\includegraphics[width=0.85\columnwidth]{face-swapping-process}
%\caption{Process of generating Deepfake videos.}
%\label{fig:process}
%\end{figure}
%


One of the first works on face swapping is by Bitouk~\emph{et al.}~\cite{Bitouk2008}, where the authors searched in a database for a face similar in appearance to the input face and then focused on perfecting the blending of the found face into the input image. The main motivation for this work was de-identification of an input face and its privacy preservation. Hence, the approach did not allow for a seamless swapping of any two given faces. Until the latest era of neural networks, most of the techniques for face swapping or facial reenacment were based on similarity searchers between faces or face patches in target and source video and various blending techniques~\cite{Arar2011,Xingjie2014,Uyl2015,Mahajan2017,Nirkin2018}.

The first approach that used a generative adversarial network to train a model between pre-selected two faces was proposed by Korshunova~\emph{et al.}\ in 2017~\cite{Korshunova2017}. Another related work with even a more ambitious idea was to use long short term memory (LSTM) based architecture to synthesize a mouth feature solely from an audio speech~\cite{Shlizerman2017}. Right after these publication became public, they attracted a lot of publicity. Open source approaches replicating these techniques started to appear, which resulted in the Deepfake phenomena. 

The rapid spread of Deepfakes and the ease of generating such videos are calling for a reliable detection method. So far, however, there are only few publications focusing on detecting GAN-generated videos with swapped faces and very little data for evaluation and benchmarking is publicly available. For instance, Zhang~\emph{et al.}~\cite{Zhang2017} proposed the method based on speeded up robust features (SURF) descriptors and SVM classifier. The authors evaluated this approach on a set of images where the face of one person was replaced with a face of another by applying color correction and smoothing techniques based on Gasussian blurring, which means the facial expressions of the input faces were not preserved. Another method based on LBP-like features with SVM classifier was proposed by Agarwal~\emph{et al.}~\cite{Agarwal2017} and evaluated on the videos collected by the authors with Snapchat\footnotemark[3] phone application. Snapchat uses active 3D model to swap faces in real time, so the resulted videos are not really Deepfakes, but it is still a widely used tool and database of such videos, if it will ever become public (the authors promised to release it but have not done so at the moment of publication), it can be interesting to research community. 


R\"{o}ssler~\emph{et al.}~\cite{Verdoliva2018}  presented the most comprehensive database of non-Deepfake swapped faces ($500'000$ images from more than $1000$ videos)  to date. The authors also benchmarked the state of the art forgery classification and segmentation methods. The authors used Face2Face~\cite{Thies2016} tool to generate the database, which is based on expression transformation using 3D facial model and a pre-computed database of mouth interiors. 
%The authors further improved the quality of face swapping using a pre-trained autoencoder. Their proposed forgery detection method based on a deep neural network could detect swapped faces with a high accuracy. 
One of the latest approaches~\cite{Li2018} proposed to use blinking detection as the means to distinguish swapped faces in Deepfake videos. The authors generated $49$ videos (not publicly available) and argued that the proposed eye blinking detection was effective in detecting Deepfake videos.


However, no public Deepfake video database where GAN-based approach was applied is available. Hence, it is unclear whether the above methods would be effective in detecting such faces. In fact, the Deepfakes that we have generated can effectively mimic the facial expressions, mouth movements, and blinking, so the current detection approaches need to be evaluated on such videos. However, it is practically impossible to evaluate the methods proposed in~\cite{Verdoliva2018} and~\cite{Li2018} as their implementations are not yet available.
%Therefore, in this paper, we present a  Deepfake video database where faces were swapped using GAN-based approach. It should be also noted, that contrary to~\cite{Li2018}, our Deepfake videos show significant amount of blinking. 


